The Ptolemy field of $3$-manifold-representations

The Ptolemy coordinates for boundary-unipotent SL(n,C)-representations of a 3-manifold group were introduced in Garoufalidis-Thurston-Zickert inspired by the A-coordinates on higher Teichm\"{u}ller space due to Fock and Goncharov. In this paper, we define the Ptolemy field of a (generic) PSL(2,\C)-representation and prove that it coincides with the trace field of the representation. This gives an efficient algorithm to compute the trace field of a cusped hyperbolic manifold.

==> figures_gen/Test.tex <==
\begingroup
 \setlength{\unitlength}{0.8pt}
 \begin{picture}(202.94643,66.428574)
 \put(0,0){\includegraphics{figures_gen/Test_included}}

\definecolor{inkcol1}{rgb}{0.0,0.0,0.0}
   \put(57.142857,21.071421){\rotatebox{360.0}{\makebox(0,0)[tl]{\strut{}{
    \begin{minipage}[h]{111.71428pt}
\textcolor{inkcol1}{\large{$E=mc^2$}}\\
\end{minipage}}}}}%

 \end{picture}
\endgroup


==> figures_gen/wh_link_edges_and_cusps.tex <==
\begingroup
 \setlength{\unitlength}{0.8pt}
 \begin{picture}(232.4025,96.17975)
 \put(0,0){\includegraphics{figures_gen/wh_link_edges_and_cusps_included}}
 \end{picture}
\endgroup

